Provably Robust Conformal Prediction with Improved Efficiency

Conformal prediction is a powerful tool to generate uncertainty sets with guaranteed coverage using any predictive model, under the assumption that the training and test data are i.i.d.. Recently, it has been shown that adversarial examples are able to manipulate conformal methods to construct prediction sets with invalid coverage rates, as the i.i.d. assumption is violated. To address this issue, a recent work, Randomized Smoothed Conformal Prediction (RSCP), was first proposed to certify the robustness of conformal prediction methods to adversarial noise. However, RSCP has two major limitations: (i) its robustness guarantee is flawed when used in practice and (ii) it tends to produce large uncertainty sets. To address these limitations, we first propose a novel framework called RSCP+ to provide provable robustness guarantee in evaluation, which fixes the issues in the original RSCP method. Next, we propose two novel methods, Post-Training Transformation (PTT) and Robust Conformal Training (RCT), to effectively reduce prediction set size with little computation overhead. Experimental results in CIFAR10, CIFAR100, and ImageNet suggest the baseline method only yields trivial predictions including full label set, while our methods could boost the efficiency by up to $4.36\times$, $5.46\times$, and $16.9\times$ respectively and provide practical robustness guarantee. Our codes are available at https://github.com/Trustworthy-ML-Lab/Provably-Robust-Conformal-Prediction.

==> Tab/Tab_cifar_clean.tex <==
\begin{table*}[!h]
\centering
\scalebox{0.88}{
\begin{tabular}{l|p{1cm}c|p{1cm}c|p{1cm}c|p{1cm}c}
 &   \multicolumn{4}{c|}{CIFAR10}                  &          \multicolumn{4}{c}{CIFAR100}        \\ \hline
                &   \multicolumn{2}{c}{APS}                  &          \multicolumn{2}{c|}{HPS}         &   \multicolumn{2}{c}{APS}                  &          \multicolumn{2}{c}{HPS}                  \\ \hline
Method          & Coverage & Average size $\downarrow$ & Coverage & Average size $\downarrow$ & Coverage & Average size $\downarrow$ & Coverage & Average size $\downarrow$  \\ \midrule
Baseline       & 96.58\%  &   2.621         & 95.37\%  &            2.008 &  95.17\% & 15.78       &  95.11\%  & 13.94       \\
 \midrule
PTT (Ours)        & 93.48\%  & 2.094 (-20.11\%) & 93.26\%  &   \textbf{1.700 (-15.34\%)}  &   93.26\% & 12.44 (-21.17\%)        & 93.09\%   & 10.49 (-24.75\%)            \\
RCT (Ours)         & 95.02\%  & 2.158 (-17.67\%)  &   93.79\%       & 1.837 (-8.52\%)  &  94.84\% & 15.26 (-3.30\%)       & 94.71\% & 13.56 (-2.76\%)    \\
PTT + RCT (Ours)  & 93.67\%   & \textbf{1.815 (-30.75\%)} &   93.59\%       & 1.783 (-11.21\%) &  93.06\% & \textbf{12.03 (-23.76\%)}       & 92.92\%  & \textbf{10.36 (-25.68\%)}  
\end{tabular}
}
\caption{\textbf{Coverage and average prediction set size results on CIFAR 10 and CIFAR 100 \cite{krizhevsky2009learning}.} We exhibit the coverage and average size on \textbf{clean examples}. $\epsilon=0.125$, $\sigma=0.5$ and $1-\alpha=0.9$ are chosen. We compare the results for vanilla RSCP (Baseline), post-training transformation (PTT), robust conformal training (RCT) and the combination of two methods (PTT+RCT). The improvement relative to baseline is shown in parentheses and the best results are bold. }
\label{tab:cifar_clean}
\end{table*}

==> Tab/Tab_imagenet_clean.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{l|p{1cm}l|p{1cm}l}
                &           \multicolumn{2}{c}{APS}                &         \multicolumn{2}{c}{HPS}              \\ \hline
Method          & Coverage & Average size $\downarrow$ & Coverage & Average size $\downarrow$ \\ \midrule
Baseline        &  96.02\%        & 49.50       &   95.06\%       & 16.06      \\
PTT (Ours)         &   92.30\%       & 28.86 (-41.70\%)        &   91.70\%     & 8.24 (-48.69\%)      \\
\end{tabular}
\caption{\textbf{Coverage and average set size results for ImageNet \cite{deng2009imagenet}.} Results are presented on \textbf{clean examples} and $\epsilon=0.25$, target coverage $1-\alpha=0.9$ and $\sigma=0.5$ are chosen for RSCP. Vanilla RSCP (Baseline) and post-training transformation (PTT) are compared. The improvement relative to baseline is shown in parentheses.}
\label{tab:imagenetClean}
\end{table*}

==> Tab/tab_RSCPplus.tex <==
\begin{table}[b]
\centering
\scalebox{0.95}{
\begin{tabular}{l|l|l|l|l|l|l}
\hline
Base score      & \multicolumn{3}{c|}{HPS} &  \multicolumn{3}{c}{APS}                                                    \\ \hline
Dataset         & CIFAR10     & CIFAR100    & ImageNet  & CIFAR10     & CIFAR100    & ImageNet\\ \hline
Baseline  & 10       & 100    & 1000    &10&100& 1000 \\ \cite{gendler2021adversarially} &&&&&&\\ 
PTT \textbf{(Ours)}        &\textbf{2.152}&23.47& \textbf{58.09}   & 2.675 & 21.77& \textbf{84.72}\\ 
% RCT(Ours)       & 10      & 100   & -     &10&100& - \\ 
PTT+RCT \textbf{(Ours)}    &\textbf{2.152}&\textbf{16.66}& -       & \textbf{2.576} & \textbf{19.25}& -\\ \hline
\end{tabular}
}
\caption{\textbf{Average size of \algoname~on three vision datasets.} Results are derived with $\beta=10^{-3}$ and $N_{\text{MC}}=256$ Monte Carlo samples. For CIFAR10 and CIFAR100, $\epsilon=0.125$ and $\sigma=0.25$. For ImageNet, $\epsilon=0.25$ and $\sigma=0.5$. Following \cite{gendler2021adversarially}, we take $N_{\text{split}} = 50$ random splits between calibration set and test set and present the average results(Same for \cref{tab:cifar,tab:imagenet}). The standard deviation is reported in \cref{app:cleanResult}. We could see that the baseline method only gives trivial predictions containing the whole label set, while with PTT or PTT + RCT we can give informative \& compact predictions. }
\label{tab:RSCPplusMain}
\end{table}

==> src/algorithm.tex <==
\begin{minipage}{0.66\textwidth}
\begin{algorithm}[H]
\caption{\algoname: Generate provably robust prediction set. }
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Input image $\testx$, calibration set $D_{cal}$, target coverage level $1 - \alpha$, $\epsilon$, $\sigma$, $\beta$}
\Output{Guaranteed robust prediction set $C_\epsilon^+$}
Calculate calibration scores with randomized smoothing$\{\hat{S}_{\text{RS}}(x, y)\}_{(x, y) \in D_{\text{cal}}}$\;
Calculate threshold $\tau_{\text{MC}}$ as $\frac{1 - \alpha - 2\beta}{1 + 1 / |D_{\text{cal}}|}$ empirical quantile of  calibration scores\;
Calculate test conformity score for each class with randomized smoothing ${\hat{S}_{\text{RS}}(\tilde{x}_{n+1}, k)}_{k=1}^K$\;
Calculate prediction set $C_\epsilon^+$ with \cref{eq:RSCP+Pred}.
\end{algorithm}
\end{minipage}

